OPSurv: Orthogonal Polynomials Quadrature Algorithm for Survival Analysis

This paper introduces the Orthogonal Polynomials Quadrature Algorithm for Survival Analysis (OPSurv), a new method providing time-continuous functional outputs for both single and competing risks scenarios in survival analysis. OPSurv utilizes the initial zero condition of the Cumulative Incidence function and a unique decomposition of probability densities using orthogonal polynomials, allowing it to learn functional approximation coefficients for each risk event and construct Cumulative Incidence Function estimates via Gauss--Legendre quadrature. This approach effectively counters overfitting, particularly in competing risks scenarios, enhancing model expressiveness and control. The paper further details empirical validations and theoretical justifications of OPSurv, highlighting its robust performance as an advancement in survival analysis with competing risks.

==> sections/discussion.tex <==
\section{Discussion}
% \lilian{TODO: can someone please help write this section?}


% \tristan{LATER BUT REALLY GOOD TO HAVE: (examine generalizability) remove data and examine how performance changes in the reduction of training data. A simple plot would be good. Just do one-pass for this section. Get results quick.}

\subsection{Survival and cumulative incidence functions} \label{survCIF}
% \lilian{PLEASE REVIEW}
Given that OPSurv differs from existing methods in its functional-analytic approach to modeling, we provide plots of the Survival functions and CIFs to help the reader visualize our model outputs. Figures~\ref{fig:metabric_surv_func} and \ref{fig:seer_surv_event_1} show the survival curves of 3 randomly selected patients from the METABRIC dataset and the SEER data set who died from the primary cause, respectively. In particular, the times of death seemed to have happened at the time preceding a sharp decline of the survival function.

\begin{figure*}[h]
\vspace{-0.2cm}
\includegraphics[width=.9\textwidth]{figures/METABRIC_surv_func.pdf}
  \centering
  \vspace{-2.5mm}
  \caption{METABRIC: Survival functions of the six models for three random test patients. The x-axis is observation time (25 years). Vertical lines indicate the times of death for each patient. Observe that the times of death preceded the sudden drop in all three OPSurv survival curves. \lilian{TODO: please review}}
  \label{fig:metabric_surv_func}
  % \vspace{-4mm}
\end{figure*}

\begin{figure*}[h]
\vspace{-0.2cm}
\includegraphics[width=.9\textwidth]{figures/SEER_Surv_event_1.pdf}
  \centering
  \vspace{-2.5mm}
  \caption{SEER: Survival functions of four deep learning-based models for three random test patients on the SEER dataset who experienced death from breast cancer, the primary risk. The x-axis is observation time (25 years). Times of death of the patients are indicated by the dotted vertical lines.}
  \label{fig:seer_surv_event_1}
  \vspace{-4mm}
\end{figure*}

The CIFs for 3 randomly selected patients from the SEER data set who died of the primary cause are presented in Figure~\ref{fig:seer_cif_event_1}.

\begin{figure*}[h]
\vspace{-0.2cm}
\includegraphics[width=.95\textwidth]{figures/SEER_CIF_event_1.pdf}
  \centering
  \vspace{-2.5mm}
  \caption{Cumulative incidence functions of six models for three random test patients from the SEER dataset who experienced death from the primary cause, breast cancer. The x-axis is observation time (25 years). Vertical lines indicate the time each patient experiences the event. Times of death are indicated by the dotted vertical lines.}
  \label{fig:seer_cif_event_1}
  \vspace{-1mm}
\end{figure*}

%{figures/SEER_Surv_event_1.pdf}{figures/SEER_CIF_event_1.pdf}


\begin{figure*}[h]
\vspace{-0.2cm}
\includegraphics[width=.9\textwidth]{figures/FM_Split_I_Surv_event_2.pdf}
  \centering
  \vspace{-2.5mm}
  \caption{Freddie Mac Split I: Survival functions of four deep learning-based models for three random test records on the Freddie Mac Split I dataset who experienced 60-day delinquency, the primary risk. The x-axis is observation time (48 months). Times of the event of the records are indicated by the dotted vertical lines.}
  \label{fig:fm_split_I_surv_event_2}
  \vspace{-1mm}
\end{figure*}

\begin{figure*}[h]
\vspace{-0.2cm}
\includegraphics[width=.95\textwidth]{figures/FM_Split_I_CIF_event_2.pdf}
  \centering
  \vspace{-2.5mm}
  \caption{Cumulative incidence functions of six models for three random test records from the Freddie Mac Split I dataset who experienced 60-day delinquency, the primary risk. The x-axis is observation time (48 months). Vertical lines indicate the time each patient experiences the event. Times of the event are indicated by the dotted vertical lines.}
  \label{fig:fm_split_I_cif_event_2}
  \vspace{-1mm}
\end{figure*}


